Conformal invariants measuring the best constants for Gagliardo-Nirenberg-Sobolev inequalities

We introduce a family of conformal invariants associated to a smooth metric measure space which generalize the relationship between the Yamabe constant and the best constant for the Sobolev inequality to the best constants for Gagliardo-Nirenberg-Sobolev inequalities $\|w\r|_q \leq C\|\nabla w\|_2^\theta \|w\|_p^{1-\theta}$. These invariants are constructed via a minimization procedure for the weighted scalar curvature functional in the conformal class of a smooth metric measure space. We then describe critical points which are also critical points for variations in the metric or the measure. When the measure is assumed to take a special form --- for example, as the volume element of an Einstein metric --- we use this description to show that minimizers of our invariants are only critical for certain values of $p$ and $q$. In particular, on Euclidean space our result states that either $p=2(q-1)$ or $q=2(p-1)$, giving a new characterization of the GNS inequalities whose sharp constants were computed by Del Pino and Dolbeault.

==> bg/tractor_genl.tex <==
\subsection{Basic Aspects of the Tractor Calculus}
\label{sec:bg/tractor}

Note that, in making our definition of a smooth metric measure space, we have in fact defined an object which is naturally an object in conformal geometry --- simply consider the equivalence class of triples~\eqref{eqn:scms} under the relation $(g,v^m\dvol)\sim(e^{2s}g,e^{(m+n)s}v^m\dvol)$ for any $s\in C^\infty(M)$.  In this way, by regarding the best constant in the GNS inequalities~\eqref{eqn:gns_dd} as a natural conformal invariant of a smooth metric measure space, we can hope to bring the full force of conformal something or another to bear on our problem.  For the purposes of this article, the tools we are most interested are those coming from the tractor calculus.

Roughly speaking, the tractor calculus is to conformal geometry what the tensor calculus is to Riemannian geometry.  The tractor calculus is built upon the study of a family of vector bundles, termed tractor bundles, which come equipped with metrics and connections which are canonically associated to a conformal class (cf.\ the Levi-Civita connection in Riemannian geometry).  In this way, many natural structures in conformal geometry are encoded as preferred sections of some tractor bundle.  For example, in a generalized sense which we describe below, Einstein metrics are equivalent to parallel sections of the so-called standard tractor bundle, and constant scalar curvature metrics are equivalent to a special class of constant-length sections of the standard tractor bundle.  As we will see, these conditions are quite strong, and will provide us the means to understand the GNS inequalities~\eqref{eqn:gns_dd} using conformal geometry.

One way to realize a conformal class $c$ on a manifold is as a ray subbundle $c\subset S^2T^\ast M$.  In this way, metrics in the conformal class are sections of $c$.  Moreover, there is a natural $\bR^+$ action on $c$, corresponding to pointwise conformal change of metrics, which makes $\mQ$ into a principal $\bR^+$-bundle.  This perspective gives rise to a family of important line bundles on a conformal manifold.

\begin{defn}
Let $(M^n,c)$ be a conformal manifold.  The \emph{conformal density bundle of weight $w$} is the line bundle $E[w]$ associated to $c$ via the representation $\bR\ni \rho\mapsto ?\in\bR=\End{\bR^+}$.  We will denote by $\mE[w]$ the space of smooth sections of $E[w]$.  A \emph{conformal density of weight $w$} is a section $\sigma\in\mE[w]$.
\end{defn}

In particular, if $\sigma\in\Gamma(E[w])$ and $g,h=e^{2s}g$ are two metrics in the conformal class $c$, then
\[ \sigma\left(e^{2s}g,x\right) = e^{2s(x)}\sigma(g,x) . \]
Thus, conformal densities can be thought of as functions on a manifold which scale with the metric in a particular way.  Note also that, since $\dvol(e^{2s}g)=e^{ns}\dvol(g)$, conformal densities are equivalent to use tensor densities, except that we have changed our convention in defining the weight.

A choice of a conformal class imparts further structure than just a principal $\bR^+$-bundle.  Indeed, it is clear that a conformal class $c$ gives a reduction of the frame bundle of the tangent bundle to the conformal group $\CO(n)$ of frames which are orthonormal for some choice of metric in $c$.  However, this bundle only accounts for first order data, and so we do something.  Having done this, one then arrives a canonical bundle termed the standard tractor bundle which, like the tangent bundle in the tensor calculus, forms the basis for the tractor calculus.

\begin{defn}
Let $(M^n,c)$ be a conformal manifold.  The tractor bundle $T$ is the rank $n+2$ vector bundle associated to $\bR^n$ with the properties that
\begin{enumerate}
\item For a choice of metric $g\in c$, there is an isomorphism $T\cong\bR\oplus TM\oplus\bR$, which we shall denote by
\begin{equation}
\label{eqn:tractor_coordinates}
I_g = \begin{pmatrix}\sigma\\\omega\\\rho\end{pmatrix}
\end{equation}
for each section $I\in\Gamma(T)=:\mT$.
\item For another choice of metric $h=e^{2s}g\in c$, the isomorphism~\eqref{eqn:tractor_coordinates} transforms according to
\begin{equation}
\label{eqn:tractor_law}
I_h = \begin{pmatrix} e^s\sigma\\e^{-s}(\omega+\sigma\nabla s)\\e^{-s}(\rho-g(\omega,\nabla s)-\frac{1}{2}\lv\nabla s\rv^2\sigma)\end{pmatrix} ,
\end{equation}
where $\nabla s$ and its length are computed with respect to $g$.
\end{enumerate}
\end{defn}

In particular, note that the topmost nonvanishing term in the ``coordinates'' \eqref{eqn:tractor_coordinates} is conformally invariant.  For our purposes, this is reflected in a certain canonical tractor.

\begin{defn}
Let $(M^n,c)$ be a conformal manifold.  The \emph{projector tractor} $X\in\mT[1]$ is the tractor given by
\[ X = \begin{pmatrix}0\\0\\1\end{pmatrix} \]
for any choice of scale $g\in c$.
\end{defn}

The importance of the standard tractor bundle is that it inherits a canonical metric and connection.

\begin{defn}
Let $(M^n,c)$ be a conformal manifold and let $\mT$ be the standard tractor bundle.  The \emph{tractor metric} $h\in\mT^\ast\otimes\mT^\ast$ and the \emph{canonical tractor connection} $\nabla\colon\mT\to T^\ast M\otimes\mT$ are given in a choice of scale $g\in c$ by
\begin{align*}
h\left(\begin{pmatrix}\sigma_1,\omega_1,\rho_1\end{pmatrix},\begin{pmatrix}\sigma_2,\omega_2,\rho_2\end{pmatrix}\right) & = g(\omega_1,\omega_2) + \sigma_1\rho_2 + \sigma_2\rho_1 \\
\nabla_x \begin{pmatrix}\sigma\\\omega\\\rho\end{pmatrix} & = \begin{pmatrix}\nabla_x\sigma-g(x,\omega)\\\nabla_x\omega+\sigma P(x)+\rho x\\\nabla_x\rho - P(x,\omega)\end{pmatrix} ,
\end{align*}
where $P=\frac{1}{n-2}\left(\Ric-\frac{1}{2(n-1)}Rg\right)$ is the \emph{Schouten tensor}.
\end{defn}

\begin{remark}

It is clear that the projector tractor $X$ gives an includion $\mE[-1]\hookrightarrow\mT$ via $\rho\mapsto X\otimes\rho$.  Using the tractor metric $h$, we also see that $X$ gives a projection $\mT\to\mE[1]$ via $I\mapsto h(X,I)$.
\end{remark}

\begin{remark}

We will frequently use brackets $\lp\,,\,\rp$ to denote the tractor metric $h$ when it cannot be confused with another metric.  Similarly, we will frequently denote the corresponding norm by $\lv\,\lv$.
\end{remark}

From the standpoint of parabolic geometry, the canonical tractor connection is induced by the Cartan connection on ??  Alternatively, $\nabla$ can be canonically defined via a certain cohomological condition on $H^\ast(M,\kg)$ (cf.\ \cite{CapSlovak2009}).  This latter description also gives rise to an important operator relating a particular density bundle to the standard tractor bundle.

\begin{defn}
Let $(M^n,c)$ be a conformal manifold.  The \emph{BGG splitting operator} $L\colon\mE[1]\to\mT$ is the given in a choice of scale $g\in c$ by
\[ L\sigma = \begin{pmatrix}\sigma\\\nabla\sigma\\-\frac{1}{n}(\Delta\sigma+\frac{1}{2(n-1)}R\sigma)\end{pmatrix} . \]
\end{defn}

\begin{remark}

Note that our definitions of $u$ and $v$ in Section~\ref{sec:bg/smms} are such that they can be realized as conformal densities of weight one.  In particular, we may study these functions as tractors by considering $Lu$ and $Lv$, respectively.
\end{remark}

The BGG splitting operator encodes a lot of information about the underlying conformal manifold.  For example, it can be used to test whether a metric in a conformal class has constant scalar curvature, or even if it is Einstein.

\begin{prop}[\cite{Gover2008}]
Let $(M^n,c)$ be a conformal manifold.  Given $\sigma\in\mE[1]$, the metric $\sigma^{-2}c$, where defined,
\begin{enumerate}
\item has scalar curvature $R(\sigma^{-2}c)=-n(n-1)\lv L\sigma\rv^2$, and moreover,
\item is Einstein if and only if $\nabla(L\sigma)=0$.
\end{enumerate}

Moreover, if $I\in\mT$ is parallel, then there is a $\sigma\in\mE[1]$ such that $I=L\sigma$.
\end{prop}

That $L\sigma$ is parallel if $\sigma^{-2}c$ is an Einstein metric follows from the following algebraic lemma which will be of use to us.

\begin{lem}
\label{lem:prolongation}
Let $(M^n,c)$ be a conformal manifold and let $I\in\mT$ be such that $\nabla I=\alpha\otimes X$ for some one-form $\alpha$.  Then $\alpha=0$.
\end{lem}

That there is a close relationship between Einstein metrics in a conformal class and parallel sections of the standard tractor bundle is the main reason we have introduced the tractor calculus here: so long as we choose the right form to express a function realizing equality in a GNS inequality, it will be immediately obvious when it can be of the form $(1+\lv x\rv^2)^k$ for some exponent $k$ (see Section~\ref{sec:qe}).  This is because the space of parallel tractors is finite dimensional, and on Euclidean space $(\bR^n,g_0)$, is spanned by the tractors
\[ \left\{ L(\frac{1+r^2}{2}), L(x^1), \dotsc, L(x^n), L(\frac{1-r^2}{2}) \right\} , \]
where $r$ denotes the distance from a fixed origin, $x^1,\dotsc,x^n$ are Cartesian coordinates about that origin, and our choice of basis is orthonormal, with $L(\frac{1+r^2}{2})$ having length $-1$ and the other tractors having length $1$.

To facilitate our discussion of the GNS inequalities using smooth metric measure spaces, the following computation from~\cite{Case2011t} will be useful.

\begin{prop}
\label{prop:smms_tractor_formulae}
Let $(M^n,g,v^m\dvol)$ be a smooth metric measure space and let $u$ determine a pointwise conformal change as in ??  Then it holds that
\begin{align*}
\left(\Ric_{f,\phi}^m\right)_0 & = (m+n-2)v\nabla(Lu) - mu\nabla(Lv) \\
& \quad - \frac{1}{n}\left((m+n-2)\lp\nabla(Lu),Lv\rp-m\lp\nabla(Lv),Lu\rp\right)X \\
R_{f,\phi}^m-m\Delta_\rho\beta & = -(m+n-1)nu^{-2}\lv Lu\rv^2 + mn(uv)^{-1}\lp Lu,Lv\rp \\
R_{f,\phi}^m-(m+n)\Delta_\rho\beta & = -(m+n-2)n(uv)^{-1}\lp Lu,Lv\rp + (m-1)nv^{-2}\lv Lv\rv^2 .
\end{align*}
\end{prop}
